Object Manipulation in Marine Environments using Reinforcement Learning

Performing intervention tasks in the maritime domain is crucial for safety and operational efficiency. The unpredictable and dynamic marine environment makes the intervention tasks such as object manipulation extremely challenging. This study proposes a robust solution for object manipulation from a dock in the presence of disturbances caused by sea waves. To tackle this challenging problem, we apply a deep reinforcement learning (DRL) based algorithm called Soft. Actor-Critic (SAC). SAC employs an actor-critic framework; the actors learn a policy that minimizes an objective function while the critic evaluates the learned policy and provides feedback to guide the actor-learning process. We trained the agent using the PyBullet dynamic simulator and tested it in a realistic simulation environment called MBZIRC maritime simulator. This simulator allows the simulation of different wave conditions according to the World Meteorological Organization (WMO) sea state code. Simulation results demonstrate a high success rate in retrieving the objects from the dock. The trained agent achieved an 80 percent success rate when applied in the simulation environment in the presence of waves characterized by sea state 2, according to the WMO sea state code

==> Results_and_discussion.tex <==
TBD

==> chapters/backup.tex <==

% \section{Units}

% Use SI as primary units. Other units may be used as secondary units
% (in parentheses). This applies to papers in data storage. For example,
% write ``$15\,\mathrm{Gb}/\mathrm{cm}^2$ ($100\,\mathrm{Gb}/\mathrm{in}^2$)''. 
% An exception is when
% English units are used as identifiers in trade, such as ``3.5 in
% disk drive''. Avoid combining SI and other units, such as current in
% amperes and magnetic field in oersteds. This often leads to confusion
% because equations do not balance dimensionally. If you must use mixed
% units, clearly state the units for each quantity in an equation.  The
% SI unit for magnetic field strength $\mathbf{H}$ is $\mathrm{A}/\mathrm{m}$. However, if you wish to
% use units of $\mathrm{T}$, either refer to magnetic flux density $\mathbf{B}$ or
% magnetic field strength symbolized as $\mu_0\,\mathbf{H}$. Use the center dot to
% separate compound units, e.g., ``$\mathrm{A} \cdot \mathrm{m}^2$''.

% \section{Helpful Hints}

% \subsection{Figures and Tables}

% Figure axis labels are often a source of confusion. Use words rather
% than symbols. As an example, write the quantity ``Magnetization'', or
% ``Magnetization M'', not just ``M''. Put units in parentheses. Do not
% label axes only with units.  For example, write ``Magnetization
% ($\mathrm{A}/\mathrm{m}$)'' or ``Magnetization ($\mathrm{A} \mathrm{m}^{-1}$)'', not just
%  ``$\mathrm{A}/\mathrm{m}$''. Do not
% label axes with a ratio of quantities and units. For example, write
% ``Temperature ($\mathrm{K}$)'', not ``$\mbox{Temperature}/\mathrm{K}$''.

% Multipliers can be especially confusing. Write ``Magnetization
% ($\mathrm{kA}/\mathrm{m}$)'' or ``Magnetization ($10^3 \mathrm{A}/\mathrm{m}$)''. Do not write
% ``Magnetization $(\mathrm{A}/\mathrm{m}) \times 1000$'' because the reader would not know
% whether the axis label means $16000\,\mathrm{A}/\mathrm{m}$ or $0.016\,\mathrm{A}/\mathrm{m}$.

% \subsection{References}

% Use Harvard style references (see at the end of this document). With
% \LaTeX, you can process an external bibliography database 
% using \texttt{bibtex},\footnote{In this case you will also need the \texttt{ifacconf.bst}
% file, which is part of the \texttt{ifaconf} package.}
% or insert it directly into the reference section. Footnotes should be avoided as
% far as possible.  Please note that the references at the end of this
% document are in the preferred referencing style. Papers that have not
% been published should be cited as ``unpublished''.  Capitalize only the
% first word in a paper title, except for proper nouns and element
% symbols.

% \subsection{Abbreviations and Acronyms}

% Define abbreviations and acronyms the first time they are used in the
% text, even after they have already been defined in the
% abstract. Abbreviations such as IFAC, SI, ac, and dc do not have to be
% defined. Abbreviations that incorporate periods should not have
% spaces: write ``C.N.R.S.'', not ``C. N. R. S.'' Do not use abbreviations
% in the title unless they are unavoidable (for example, ``IFAC'' in the
% title of this article).

% \subsection{Equations}

% Number equations consecutively with equation numbers in parentheses
% flush with the right margin, as in (\ref{eq:sample}).  To make your equations more
% compact, you may use the solidus ($/$), the $\exp$ function, or
% appropriate exponents. Use parentheses to avoid ambiguities in
% denominators. Punctuate equations when they are part of a sentence, as
% in

% \begin{equation} \label{eq:sample2}
% \begin{array}{ll}
% \int_0^{r_2} & F (r, \varphi ) dr d\varphi = [\sigma r_2 / (2 \mu_0 )] \\
% & \cdot \int_0^{\inf} exp(-\lambda |z_j - z_i |) \lambda^{-1} J_1 (\lambda  r_2 ) J_0 (\lambda r_i ) d\lambda 
% \end{array}
% \end{equation}

% Be sure that the symbols in your equation have been defined before the
% equation appears or immediately following. Italicize symbols ($T$
% might refer to temperature, but T is the unit tesla). Refer to
% ``(\ref{eq:sample})'', not ``Eq. (\ref{eq:sample})'' or ``equation
% (\ref{eq:sample})'', except at the beginning of a sentence: ``Equation
% (\ref{eq:sample}) is \ldots''.

% \subsection{Other Recommendations}

% Use one space after periods and colons. Hyphenate complex modifiers:
% ``zero-field-cooled magnetization''. Avoid dangling participles, such
% as, ``Using (1), the potential was calculated'' (it is not clear who or
% what used (1)). Write instead: ``The potential was calculated by using
% (1)'', or ``Using (1), we calculated the potential''.

% A parenthetical statement at the end of a sentence is punctuated
% outside of the closing parenthesis (like this). (A parenthetical
% sentence is punctuated within the parentheses.) Avoid contractions;
% for example, write ``do not'' instead of ``don' t''. The serial comma
% is preferred: ``A, B, and C'' instead of ``A, B and C''.










% bib file to produce the bibliography
                                                     % with bibtex (preferred)
                                                   
%\begin{thebibliography}{xx}  % you can also add the bibliography by hand

%\bibitem[Able(1956)]{Abl:56}
%B.C. Able.
%\newblock Nucleic acid content of microscope.
%\newblock \emph{Nature}, 135:\penalty0 7--9, 1956.

%\bibitem[Able et~al.(1954)Able, Tagg, and Rush]{AbTaRu:54}
%B.C. Able, R.A. Tagg, and M.~Rush.
%\newblock Enzyme-catalyzed cellular transanimations.
%\newblock In A.F. Round, editor, \emph{Advances in Enzymology}, volume~2, pages
%  125--247. Academic Press, New York, 3rd edition, 1954.

%\bibitem[Keohane(1958)]{Keo:58}
%R.~Keohane.
%\newblock \emph{Power and Interdependence: World Politics in Transitions}.
%\newblock Little, Brown \& Co., Boston, 1958.

%\bibitem[Powers(1985)]{Pow:85}
%T.~Powers.
%\newblock Is there a way out?
%\newblock \emph{Harpers}, pages 35--47, June 1985.

%\bibitem[Soukhanov(1992)]{Heritage:92}
%A.~H. Soukhanov, editor.
%\newblock \emph{{The American Heritage. Dictionary of the American Language}}.
%\newblock Houghton Mifflin Company, 1992.

%\end{thebibliography}

% \appendix
% \section{A summary of Latin grammar}    % Each appendix must have a short title.
% \section{Some Latin vocabulary}              % Sections and subsections are supported  
%                                                                          % in the appendices.




% \subsection{Tables}
% Tables must be centered and have a caption above them, numbered with
% Arabic numerals. See table~\ref{tb:margins} for an example.

% \begin{table}[hb]
% \begin{center}
% \caption{Margin settings}\label{tb:margins}
% \begin{tabular}{cccc}
% Page & Top & Bottom & Left/Right \\\hline
% First & 3.5 & 2.5 & 1.5 \\
% Rest & 2.5 & 2.5 & 1.5 \\ \hline
% \end{tabular}
% \end{center}
% \end{table}

% \subsection{Final Stage}

% Authors are expected to mind the margins diligently.  Papers need to
% be stamped with event data and paginated for inclusion in the
% proceedings. If your manuscript bleeds into margins, you will be
% required to resubmit and delay the proceedings preparation in the
% process.

% \subsubsection{Page margins.} See table~\ref{tb:margins} for the
% page margins specification. All dimensions are in \emph{centimeters}.


% \subsection{PDF Creation}

% All fonts must be embedded/subsetted in the PDF file. Use one of the
% following tools to produce a good quality PDF file:

% \subsubsection{PDFLaTeX} is a special version of LaTeX by Han The
% Thanh which produces PDF output directly using Type-1 fonts instead of
% the standard \texttt{dvi} file. It accepts figures in JPEG, PNG, and PDF
% formats, but not PostScript. Encapsulated PostScript figures can be
% converted to PDF with the \texttt{epstopdf} tool or with Adobe Acrobat
% Distiller.

% \subsubsection{Generating PDF from PostScript} is the classical way of
% producing PDF files from LaTeX. The steps are:

% \begin{enumerate}
%   \item Produce a \texttt{dvi} file by running \texttt{latex} twice.
%   \item Produce a PostScript (\texttt{ps}) file with \texttt{dvips}.
%   \item Produce a PDF file with \texttt{ps2pdf} or Adobe Acrobat
%   Distiller.
% \end{enumerate}

% \subsection{Copyright Form}

% IFAC will put in place an electronic copyright transfer system in due
% course. Please \emph{do not} send copyright forms by mail or fax. More
% information on this will be made available on IFAC website.


==> chapters/introduction.tex <==
\section{Introduction}
%In the last decades the importance of object manipulation in maritime operations has grown tremendously, where autonomous systems are increasingly being used practical solution to global maritime security challenges such as illegal fishing, piracy, smuggling and human-trafficking[MBZIRC]. As field robotics advance beyond observation-oriented tasks towards intervention-based activities, there is an increasing imperative for control methods that demonstrate resilience in the presence of external disturbances originating from the surrounding environment. Mounting the robot arm on a mobile base adds complexity, requiring the agent to factor in its own movement during action selection. Through continuous interaction and learning, the RL agent refines its policy, enabling the mobile robot arm to master object manipulation in increasingly dynamic environments. There exist developed techniques for manipulators integrated into mobile vehicles, including autonomous underwater vehicles (AUVs) [Carlucho2020ARL] and unmanned aerial vehicles[8299552], are currently in existence. Typically, these applications are confined to scenarios with minimal water and wind disturbances. Moreover, mobile manipulators on terrestrial vehicles are generally constrained to environments featuring smooth roads and walkways. 

%Marine robotics has gained significant importance in recent years, where autonomous systems are increasingly being used as practical solutions to global maritime security challenges such as illegal fishing, piracy, smuggling and human-trafficking. Marine robots, particularly unmanned surface vessels (USVs) now require to perform not only observation-oriented tasks but also intervention-based activities. To perform these tasks in the complex and dynamic marine environment, an advanced object manipulation system that robustly retrieves object with high success rate while being resilient in the presence of external disturbances originating from the surrounding environment is required.


Marine robotics has gained significant importance in recent years, where autonomous systems are increasingly being used as practical solutions to environmental
monitoring and for maritime security challenges such as illegal fishing, piracy, smuggling, and human trafficking cite\{}\omar{some statistics? + ref}. Marine robots, particularly unmanned surface vessels (USVs) are required to perform tasks like autonomous surveillance, tracking, and intervention-based activities for manipulation. \omar{you can here motivate your task and why it is important}. To develop solutions for intervention-related tasks in the complex and dynamic marine environment, an advanced object manipulation system that robustly retrieves objects with a high success rate while being resilient in the presence of external disturbances originating from the surrounding environment is required. \textcolor{red}{Please add some references in this paragraph, e.g., the IROS paper by Marin et al. and other papers to support the tasks that are performed by the USV.}

\omar{why RL? motivate it a little bit.}
Reinforcement learning (RL) is transforming robotic tasks unlocking exciting possibilities for ever-more complex and real-world object manipulation, including grasping and placing both static and dynamic objects. In the RL framework, the robot arm control problem can be formulated as a Markov Decision Process (MDP)~\cite{Puterman1994MarkovDP}. \omar{why these details here?} Solving a RL problem consists in iteratively learning a task from interactions to achieve a goal. During learning, an artificial agent (controller) interacts with the target system (arm) by taking an action (torque command), that makes the robot evolve from its current state $x_t \in X \subseteq \mathbb{R}^n$ to $x_{t+1}$. The agent then receives a numerical signal $r_t$, called reward, which provides a measure of how good (or bad) the action taken at time $t$ is in terms of the observed state transition. Many works have used the RL paradigm for controlling manipulators attached to AUVs in underwater environment \cite{Carlucho2020ARL}. However, this technique has not yet been applied to task of manipulating objects in harsh maritime environments using RL. We utilization RL to obtain an optimal policy for successfully accomplishing the task by itself without any motion prediction of the waves by learning with experience over a wide variety of wave characteristics based on WMO Sea state code using the simulator.

In the case of mobile robots,mounting the robot arm on a mobile base adds complexity, requiring the agent to factor in its own movement during action selection. There exist developed techniques for manipulators integrated into mobile vehicles, including autonomous underwater vehicles (AUVs) \cite{Carlucho2020ARL} and unmanned aerial vehicles\cite{8299552}, are currently in existence. Typically, these applications are confined to scenarios with minimal water and wind disturbances. Moreover, mobile manipulators on terrestrial vehicles are generally constrained to environments featuring smooth roads and walkways. 

In maritime environments, especially in our case, the robotic arm is mounted on an unmanned surface vehicle which is a non-inertial platform like boats and ships, these platforms must contend with significant inertial forces arising from the platform's non-inertial motion. Conventionally, the motion of the non-inertial platform is predicted and then motion planning and control algorithms are employed to mitigate these perturbations. There exist papers that work on end effector pose stabilisation of the robot arm in the presence of ocean waves and currents \cite{Woolfrey2021PredictiveEC}\cite{5152666}, they utilize Model Predictive Control (MPC) \cite{Alamir2008ModelPC}. However, one of the drawbacks of this technique is that it requires an accurate model of the plant to work properly, not a trivial matter in maritime environments. Furthermore, they do not perform grasping of objects related tasks.  An even more efficient way would be to leverage these inertial forces to reach a target more efficiently.   



\begin{figure}
\begin{center}
%
\includegraphics[scale=0.2650]{chapters/combined01.pdf}    % The printed column width is 8.4 cm.
\caption{Training and testing environments for object manipulation. Fig-A: Pybullet training environment for object grasping. Fig-B:  shows the testing environment.} 
\label{fig:gym}
\end{center}
\end{figure}

%The core contribution of this paper is to develop a reinforcement learning agent that enables a manipulator on a moving base to grasp objects while under disturbance caused by ocean waves and currents. Our reinforcement learning formulation is based on the Soft Actor Critic algorithm \cite{pmlr-v80-haarnoja18b}. The proposed method uses an actor critic structure, where the actor is a function that maps system states to actions and the critic is a function that assess actions chosen by the actor. Deep Neural Networks (DNN) are used as function approximators for the actor and critic. Results in simulation show the advantages of our proposed technique, shown in Fig. 1. The proposed RL agent is compared with a motion planner \cite{Kuffner2000RRTconnectAE}, showing that the RL controller can achieve what the motion planner fails repeatedly to achieve. 

%\omar{this section can be itemized as 3 contributions.} 
%The core contribution of this paper is the reinforcement learning agent that trains an optimal policy for successfully accomplishing the task by itself without any motion prediction of the waves by learning with experience over a wide variety of wave characteristics based on WMO Sea state code using the simulator \cite{MBZIRC}. Results in simulation show the advantages of our proposed technique, shown in Fig. 3. The proposed RL agent is compared with a motion planner \cite{Kuffner2000RRTconnectAE}, showing that the RL controller can achieve what the motion planner fails repeatedly to achieve. 

%\omar{if you didn't find a space at the end you can remove this paragraph.} The rest of the paper is structured as follows; Section 2 presents an overview of related works followed by Section 3 that introduces the methodology and the details of our implementations, in Section 4 we present the results obtained with our proposed control scheme, and finally Section 5 presents the overall conclusions of the proposed work. 
\textcolor{red}{ doont  Pin  .}

\omar{btw, you may wanna use DGME task for the task name. Dynamic Grapsing etc..}

In summary, the key contributions of this work are:
\begin{enumerate}
    \item \omar{my suggestion: Investigate the challenge of retrieving objects from the dock, subject to wave disturbances, using a robotic arm-equipped USV.} 
    
    Enriching the literature by exploring the unique grasping challenge of retrieving objects from the dock using a USV equipped with a robotic arm while subject to wave disturbances, as Previous research primarily concentrated on stabilizing the end effector pose of the robot arm in the presence of waves, neglecting actual manipulation tasks. 
    
    \item \omar{my suggestion: Experiment with Reinforcement Learning models to carry out the DGME task. Our findings reveal that effective results can be achieved by training on grasping static objects, bypassing the need for explicitly training with wave disturbance signals.} 
    
    Using free model reinforcement learning to successfully achieve the task, which doesn’t necessitate a model of the world or any prediction of the waves, while also showing that specific dynamic training for wave disturbances is not necessary and training with randomly placed static objects can achieve good results.
    
    \item  \omar{Develop realistic test simulations for the DGME task across diverse sea conditions, following the WMO Sea State code, and conduct an in-depth comparison and analysis of the results.}
    
    Performing realistic simulation tests for the proposed method across varied sea conditions in accordance with the WMO Sea State code and subsequently conducting a thorough comparison and analysis of the obtained results.
\end{enumerate}
